Keyphrase Annotation with Graph Co-Ranking

Keyphrase annotation is the task of identifying textual units that represent the main content of a document. Keyphrase annotation is either carried out by extracting the most important phrases from a document, keyphrase extraction, or by assigning entries from a controlled domain-specific vocabulary, keyphrase assignment. Assignment methods are generally more reliable. They provide better-formed keyphrases, as well as keyphrases that do not occur in the document. But they are often silent on the contrary of extraction methods that do not depend on manually built resources. This paper proposes a new method to perform both keyphrase extraction and keyphrase assignment in an integrated and mutual reinforcing manner. Experiments have been carried out on datasets covering different domains of humanities and social sciences. They show statistically significant improvements compared to both keyphrase extraction and keyphrase assignment state-of-the art methods.

==> attic/input/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
  In this paper, we have proposed a co-ranking approach to performing keyphrase
  extraction and keyphrase assignment jointly. Our method,
  TopicCoRank, builds two graphs: one with the
  document topics and one with controlled keyphrases (training keyphrases). We
  design a strategy to unify the two graphs and rank by importance topics and
  controlled keyphrases using a co-ranking vote.
  
  We performed experiments on four datasets of different languages and
  domains. Results showed that our approach benefits from both controlled
  keyphrases and document topics, improving both keyphrase extraction and keyphrase assignment
  baselines.
  %
  TopicCoRank can be used to annotate keyphrases in the way of professional
  indexers.
  %TopicCoRank can also be adapted to more specific problems. For instance,
  %in some cases it might be interesting to assign very specific keyphrases to the
  %document, whereas in other cases it may be interesting to assign more general keyphrases. The
  %minimum depth between a controlled keyphrase and a document topic within the unified graph encodes this
  %degree of generalization. A controlled keyphrase directly connected to a
  %document topic has the lowest generalization regarding the document,
  %followed by its connected controlled keyphrases, etc.
  %
  %In future work, we plan to investigate unsupervised variants of TopicCoRank.
  %Indeed, Wikipedia or Freebase data could be used to replace training keyphrases as controlled keyphrases.

  In future work, we will explore unsupervised constructions of the domain
  graph (using Wikipedia data, bootstrapping techniques, etc.) and explore
  more complex unification strategies in order to more accurately connect the
  document and the domain graph.


==> attic/input/experimental_settings.tex <==
\section{Experimental Settings}
\label{sec:experimental_settings}
  \subsection{Datasets}
  \label{subsec:datasets}
    We conduct our experiments on four datasets: Linguistics, Archaeology, DUC
    and SemEval. They differ in terms of language, nature and size. The following
    is the description of each dataset.

    \paragraph{Linguistics} is a collection of 715 bibliographic records that we
    collected from the French digital library Inist\footnote{The dataset will
    soon be available.}. The bibliographic records
    contain abstracts of scientific papers in the Linguistics area. The
    keyphrases are annotated by professional indexers. Indexers were
    given the instruction to assign keyphrases from a controlled vocabulary and to extract new
    concepts or very specific keyphrases from the bibliographic records. We divided the
    corpus into two disjoint sets: a training set containing 515 bibliographic
    records and a test set containing 200 bibliographic records.
    
    \paragraph{Archaeology} is a collection of 718 bibliographic records that we
    also collected from the French digital library Inist\footnote{The dataset will
    soon be available.}. The bibliographic records
    contain abstracts of scientific papers in the Archaeology area. Similar to
    the Linguistics dataset, the keyphrases are annotated by professional
    indexers. We divided the corpus into two disjoint sets: a training set
    containing 515 bibliographic records and a test set containing 200
    bibliographic records.

    \paragraph{DUC~\textnormal{\cite{wan2008expandrank}}} is a collection of 308
    news articles categorized within 30 topics. The documents have been manually
    annotated by students with 0.70 of inter-agreement (Kappa). DUC has no
    training set. For each document, we use the other
    documents of its topic to build the controlled graph.

    \paragraph{SemEval~\textnormal{\cite{kim2010semeval}}} contains 244 English
    scientific papers collected from the ACM Digital Libraries (conference and
    workshop papers). The papers represent four areas of Computer Science:
    Distributed Systems; Information Search and Retrieval; Distributed
    Artificial Intelligence -- Multiagent Systems; Social and Behavioral
    Sciences -- Economics. SemEval is divided into two disjoint sets: a training
    set containing 144 documents and a test set containing 100 documents. The
    associated keyphrases are provided by both authors and readers. As we do for
    DUC, we use keyphrases annotated on training documents of the same Computer Science
    area to build the controlled graph.
    
    \begin{table*}
        \centering
        \resizebox{\linewidth}{!}{
          \begin{tabular}{l|ccc|ccc|ccc|ccc}
            \toprule
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Linguistics}} & \multicolumn{3}{c|}{\textbf{Archaeology}} & \multicolumn{3}{c|}{\textbf{DUC}} & \multicolumn{3}{c}{\textbf{SemEval}}\\
            \cline{2-13}
            & P & R & F$^{~~}$ & P & R & F$^{~~}$ & P & R & F$^{~~}$ & P & R & F\\
            \hline
            TopicRank & 11.3 & 13.1 & 12.0$^{~~}$ & 28.1 & 19.1 & 22.2$^{~~}$ & 17.8 & 22.7 & 19.7$^{~~}$ & 14.6 & 10.1 & 11.8\\
            KEA++ & 11.6 & 13.0 & 12.1$^{~~}$ & 23.5 & 16.2 & 18.8$^{~~}$ & --- & --- & ---$^{~~}$ & --- & --- & ---\\
            \hline
            TopicCoRank$_\textnormal{\textit{extr}}$ & 14.6 & 16.8 & 15.4$^{\dagger}$ & 36.4 & 24.6 & 28.7$^{\dagger}$ & 25.5 & 32.4 & 28.1$^{\dagger}$ & 15.2 & 10.6 & 12.4\\
            TopicCoRank$_\textnormal{\textit{assign}}$ & \textbf{24.9} & \textbf{28.9} & \textbf{26.4$^{\dagger}$} & \textbf{49.1} & \textbf{33.3} & \textbf{38.8}$^{\dagger}$ & 25.9 & 33.3 & 28.8$^{\dagger}$ & 11.6 & ~~8.3 & ~~9.5\\
            \hline
            TopicCoRank & 19.0 & 22.0 & 20.1$^{\dagger}$ & 39.5 & 26.6 & 31.1$^{\dagger}$ & \textbf{28.4} & \textbf{36.6} & \textbf{31.5$^{\dagger}$} & \textbf{16.4} & \textbf{11.6} & \textbf{13.4}\\
            \bottomrule
          \end{tabular}
        }
        \caption{Results of TopicCoRank and the baselines at 10 keyphrases for each datasets.
                 Precision (P), Recall (R) and F-score (F) are reported in percentages. $\dagger$ indicates
                 a significant F-score improvement over TopicRank and KEA++ at 0.001
                 level using Student’s t-test.
                 \label{tab:comparison_results}}
    \end{table*}
    
    \paragraph{}
    Table~\ref{tab:corpus_statistics} shows factual information about the
    datasets. These datasets cover different types of document. Linguistics and Archeology
    contain the shortest documents within which a sizable amount of reference
    keyphrases cannot be extracted from the content of the documents (missing keyphrases), DUC contains larger documents where
    most keyphrases can be found within the text and SemEval is composed of the largest
    documents with fewer missing keyphrases than Linguistics and Archaeology, but still more
    than DUC.

  \subsection{Preprocessing}
  \label{subsec:preprocessing}
    We apply the following preprocessing steps to each document: sentence segmentation, word tokenization and Part-of-Speech (POS)
    tagging. We perform sentence segmentation with the PunktSentenceTokenizer
    provided by the Python Natural Language ToolKit~\cite[NLTK]{bird2009nltk}.
    We tokenize the sentences into words using the NLTK TreebankWordTokenizer for
    English and the Bonsai word tokenizer\footnote{The Bonsai word tokenizer is
    a tool provided with the Bonsai PCFG-LA parser:
    \url{http://alpage.inria.fr/statgram/frdep/fr_stat_dep_parsing.html}.} for
    French. Finally, we use the Stanford POS
    tagger~\cite{toutanova2003stanfordpostagger} for English POS tagging and
    MElt~\cite{denis2009melt} for French POS tagging.

  \subsection{Baselines}
  \label{subsec:baselines}
    To show the effectiveness of our approach, we
    compare TopicCoRank with TopicRank and KEA++. We use the official KEA++
    release\footnote{\url{http://www.nzdl.org/Kea/download.html}} and apply it to
    the Linguistics and Archaeology datasets with the Inist's thesauri\footnote{The thesauri will be soon available}. For DUC and
    SemEval, thesauri are not available. We cannot apply KEA++ to DUC and SemEval.

    We also show the performance of TopicCoRank when it only extracts keyphrases
    (TopicCoRank$_\textnormal{\textit{extr}}$) and when it only assigns keyphrases
    (TopicCoRank$_\textnormal{\textit{assign}}$).
    
  \subsection{Evaluation measures}
  \label{subsec:evaluation_measures}
    To evaluate the performance of the keyphrase extraction methods, we use the
    common measures of precision (P), recall (R) and f-score (F):
    \begin{align}
        \text{P} = \frac{\text{\textit{TP}}}{\text{\textit{TP}}+\text{\textit{FP}}},\ \text{R} = \frac{\text{\textit{TP}}}{\text{\textit{TP}} + \text{\textit{FN}}},\ \text{F} = \frac{2 \text{PR}}{\text{P} + \text{R}}
    \end{align}
    where $\textnormal{\textit{TP}}$ is the total number of correctly extracted keyphrases (true positives),
    $\textnormal{\textit{FP}}$ is the total number of erroneously extracted keyphrases (false positives) and
    $\textnormal{\textit{FN}}$ is the total number of positive keyphrases that have not been extracted (false negatives).
    We cut off the extracted keyphrases at the 10 best ranking ones and perform the
    comparisons with stemmed keyphrases.
    
    Consistent with \newcite{hassan2010conundrums}, we also report the performance of
    TopicCoRank and the baselines in terms of precision-recall curves. To generate the
    curves, we vary the evaluation cut-off from 1 to the total number of
    extracted/assigned keyphrases.



==> attic/input/introduction.tex <==
\section{Introduction}
\label{sec: introduction}
  Keyphrases are words or phrases that give a synoptic picture of what is
  important within a document. They are useful in many tasks such as
  document indexing~\cite{gutwin1999keyphrasesfordigitallibraries}, text
  categorization~\cite{hulth-megyesi:2006:COLACL} or
  summarization~\cite{litvak2008graphbased}. However, most documents do not
  provide keyphrases, and the daily flow of new documents makes the manual
  keyphrase annotation impractical. As a consequence, automatic keyphrase
  annotation has received special attention in the Natural Language
  Processing (NLP) community and many different methods have been 
  proposed~\cite{hasan2014state_of_the_art}.


  The task of automatic keyphrase annotation consists in identifying the main 
  concepts, or topics, addressed in a document.
  Keyphrase annotation methods fall into two broad categories: keyphrase 
  extraction and keyphrase assignment methods.
  Keyphrase extraction methods extract the most important words or phrases
  occurring in a document, while assignment methods provide controlled 
  keyphrases from a domain-specific terminology (controlled vocabulary).

  The automatic keyphrase annotation task is often reduced to the sole 
  keyphrase extraction task.
  Unlike assignment methods, extraction methods do not require controlled 
  vocabularies that are costly to create and to maintain. 
  Furthermore, they are able to identify new concepts.
  However, extraction methods often output ill-formed or inappropriate
  keyphrases~\cite{medelyan2008smalltrainingset}, and they produce only
  keyphrases that actually occur in the document.
  %Our intuition is that keyphrase annotation must output appropriate
  %keyphrases, i.e., mostly from controlled vocabulary, and extract
  %keyphrases that represent new concepts, i.e., within the document.

  
  Observations made on manually annotated keyphrases show that human annotators both extract keyphrases from the content of the document and
  assign keyphrases based on their knowledge of the domain~\cite{liu2011vocabularygap}. Here, we
  propose an approach that mimics this behavior and jointly extracts and assigns keyphrases.
  We use two graph representations, one for the document and one for the domain, and apply a co-ranking algorithm to perform both keyphrase extraction and assignment in a mutual reinforcing manner.
  %
  %We automatically allow this behavior by
  %unifying a graph representing reference keyphrases of a document's specific
  %domain to another graph representing keyphrase candidates selected from its
  %content. The first graph contains potential keyphrases that can be assigned,
  %while the second graph contains the potential keyphrases that can be extracted.
  %Then, we apply a co-ranking algorithm to infer the most important keyphrases.
  %
  %This paper presents a new keyphrase annotation method that uses a
  %unified-graph to represent the context of a document and its specific
  %domain, then applies a co-ranking algorithm to extract and assign the
  %keyphrases in a collaborative manner.
  
  Along with this approach come two contributions.
  First, we propose a reproducible extension to graph-based keyphrase
  extraction methods for assigning keyphrases. Second, we circumvent the need of controlled vocabulary by leveraging the reference keyphrases from training
  data.
%
%  In this work, we present a graph co-ranking approach to keyphrase 
%  annotation that simultaneously performs keyphrase assignment and 
%  extraction in a mutually reinforcing manner.
%  We rely on documents annotated with keyphrases to build a co-occurrence 
%  graph representation of the controlled vocabulary.
%  A second co-occurrence graph is built from the document and connected 
%  to the latter.
%  Keyphrase candidates extracted from the document and entries 
%  from the controlled vocabulary are then simultaneously ranked.
%  \ANNOTATE{Our assumption is that there is a mutually reinforcing relationship between
%  the ranking of the keyphrases in the document and the ranking of
%  the entries in the controlled vocabulary.}{More details to show our originality}

  We perform experiments on four datasets of different languages and domains.
  Results show that our co-ranking approach significantly improves performance over state-of-the-art approaches.

  The rest of this paper is organized as follows. Section~\ref{sec:related_work}
  presents the previous work on automatic keyphrase annotation,
  section~\ref{sec:topicrankpp} describes our method,
  section~\ref{sec:experimental_settings} presents our experimental settings and
  section~\ref{sec:results} discusses the results.
  Finally, section~\ref{sec:conclusion} concludes and shows some directions 
  for future work.


==> attic/input/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
  \subsection{Keyphrase extraction}
  \label{subsec:ake}
    Keyphrase extraction is the common approach to tackle the automatic
    keyphrase annotation task. Previous work proposed many approaches,
    including binary classification, statistical ranking and graph-based
    ranking of keyphrase candidates. As our approach uses graph-based
    ranking, we focus on the latter. For a detailed overview of
    keyphrase extraction methods, refer to~\cite{hassan2010conundrums,hasan2014state_of_the_art}.
    
    Since the seminal work of \newcite{mihalcea2004textrank}, graph-based
    ranking approaches to keyphrase extraction are becoming increasingly popular.
    The %basic plutot original dans le sens "originelle"
    original idea behind these approaches is to build a graph from 
    the input document and rank its nodes according to their importance 
    using centrality measures.
    
    In TextRank~\cite{mihalcea2004textrank}, the input document is represented as
    a co-occurrence graph in which nodes are words.
    Two words are connected by an edge if they co-occur in a fixed-sized window of words.
    A random walk algorithm is used to iteratively rank the words, then generate the
    keyphrases by concatenating the most important words.
    
    The random walk algorithm simulates the ``voting concept'', or recommendation: a node is 
    important if it is connected to many other nodes, and if many of those are 
    important.
    Thus, let $G=(V,E)$ be an undirected graph with a set of vertices $V$ and a 
    set of edges $E$, and let $E(v_i)$ be the set of nodes connected to node $v_i$.
    The score $S(v_i)$ of a vertex $v_i$ is computed iteratively until convergence 
    using the following equation:
    \begin{align}
      S(v_i) = (1 - \lambda) + \lambda \sum_{v_j \in E(v_i)}{\frac{S(v_j)}{|E(v_j)|}}
    \end{align}
    where $\lambda$ is a damping factor defined to $0.85$ by
    \newcite{brin1998pagerank}.
    
    \newcite{wan2008expandrank} first added edge weights to the random walk
    and further improved the graph with co-occurrence information borrowed from
    similar documents. To extract keyphrases from a document, they first look for
    five similar documents, then use them to add new edges between words within
    the graph and reinforce the weight of existing edges.
    
    \newcite{liu2010topicalpagerank} biased multiple graphs with topic
    probabilities. For each preliminary retrieved topic, a graph is biased with
    the conditional probabilities of the words given the topic. This method
    performs as many rankings as the number of topics and gives higher importance
    scores to high-ranking words for as many topics as possible. By doing so,
    \newcite{liu2010topicalpagerank} 
    increase the topic coverage provided by the extracted keyphrases.
    
    
    \newcite{zhang2013wordtopicmultirank} explored further the idea of
    \newcite{liu2010topicalpagerank}. Rather than using  multiple graphs biased by
    single topics, they added topics to graph nodes and performed co-ranking
    between words and topics. Topics are important if they are connected to
    important words and words are important if they are highly connected to important
    topics, to important words and to other words. At the end, only words are used for
    the keyphrase extraction.
    
    \newcite{bougouin2013topicrank}  introduced TopicRank, which is a method that
    clusters keyphrase candidates into topics, ranks these topics, and selects for
    each important topic one representative keyphrase.
    As our work extends that of \newcite{bougouin2013topicrank}, we present a
    detailed description of their method in section~\ref{subsec:topicrank}.
    
    Graph-based methods have been well studied in the past few years. However, none
    of the proposed approaches have considered the keyphrase assignment problem nor
    used a similar representation to analyze and leverage reference keyphrase
    relations within training data.

  \subsection{Keyphrase assignment}
  \label{subsec:aka}
    Keyphrase assignment provides coherent keyphrases for every document of a specific domain using
    controlled vocabulary. Dissimilar to keyphrase extraction, keyphrase assignment also
    aims to provide keyphrases that do not occur within the document. This task is more
    difficult than keyphrase extraction and has, therefore, seldom been employed for automatic
    keyphrase annotation.
    %
    %Automatic keyphrase assignment aims to provide coherent keyphrases for every
    %document of a specific domain. With assignment, keyphrases do not necessarily
    %occur within the documents. Its typical
    %use is the indexing of documents for
    %digital libraries.
    %Keyphrase assignment is a difficult task and has seldom been employed for automatic keyphrase annotation
    %\footnote{Furthermore, \newcite{hassan2010conundrums} explained that keyphrase assignment
    %is such a problem that some researchers remove reference keyphrases from evaluation
    %data if they do not occur within the documents.}.

    \newcite{medelyan2006kea++} proposed KEA++, a %simplified 
    shallow keyphrase assignment method.
    %refered to as automatic keyphrase indexing method by: je comprends pas ce que tu veux dire ....
    %\newcite{medelyan2008smalltrainingset} Pourquoi 2 fois la meme citation dans la meme phrase ? 
    %KEA++ selects candidate keyphrases using a domain-specific thesaurus 
     %and uses thesaurus information as classification feature of a binary classification algorithm. 
    KEA++ uses a domain-specific thesaurus to assign keyphrases to a document. First, keyphrase candidate are selected among the n-grams of the document.
    N-grams that do not match a thesaurus entry are either removed or substituted by a synonym that matches a thesaurus entry. This candidate selection approach induces a limitation of keyphrase assignment, refered to as keyphrase indexing by \newcite{medelyan2006kea++}, because it only assigns keyphrases if they occur within the document.
    Second, KEA++
    exploits the semantic relationships between keyphrase candidates within the thesaurus as the main feature of a Naive Bayes classifier.
    By leveraging a thesaurus, KEA++ achieves better performance than similar methods without a thesaurus.
    However, thesauri are not readily available for most domains and could be too general to perform accurate indexing.
    The application scenarii of KEA++ are thus restricted.

    %\textcolor{red}{Finalement je mettrai peut-etre une partie sur le coranking ici... je sais pas}
    
    %The study of keyphrase extraction and keyphrase assigment state-of-the-art methods shows their individual merits. 
    %Combining both methods seems promising.% subject to the condition of a consistent modelling: our basic methodology will lay on clustering 
    %and graph-based ranking methods. 
    
    \paragraph{}
    Keyphrase extraction and keyphrase assignment methods have been studied separately.
    Our work is, to our knowledge, the first attempt to perform both tasks as a distinct one.
    
    
    

%    Another notable method is the one of \newcite{liu2011vocabularygap}. They
%    proposed to recast the AKA problem as a Statistical Machine Translation
%    (SMT) problem, where document and keyphrases represent the same object in
%    two (expressively inequal) languages. By doing so, they provide keyphrases
%    that either occur or not within the document. Their experiments have
%    been conducted using title and abstract phrases instead of terminological
%    entries. This setting differs from classic AKA setting, but the assummption
%    of \newcite{liu2011vocabularygap} makes their method applicable in more
%    cases than other AKA methods.


==> attic/input/results.tex <==
\section{Results}
\label{sec:results}
  \begin{table*}
    \centering
    \resizebox{\linewidth}{!}{
      \begin{tabular}{l|ccc@{}|ccc@{}|ccc@{}|ccc@{~}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Linguistics}} & \multicolumn{3}{c|}{\textbf{Archaeology}} & \multicolumn{3}{c|}{\textbf{DUC}} & \multicolumn{3}{c}{\textbf{SemEval}}\\
        \cline{2-13}
        & P & R & F$^{~~~~}$ & P & R & F$^{~~~~}$ & P & R & F$^{~~~~}$ & P & R & F$^{~~}$\\
        \hline
        TopicRank & 11.3 & 13.1 & 12.0$^{~~~~}$ & 28.1 & 19.1 & 22.2$^{~~~~}$ & 17.8 & 22.7 & 19.7$^{~~~~}$ & 14.6 & 10.1 & 11.8$^{\ddagger}$\\
        KEA++ & 11.6 & 13.0 & 12.1$^{\dagger~~}$ & 23.5 & 16.2 & 18.8$^{~~~~}$ & --- & --- & ---$^{~~~~}$ & --- & --- & ---\\
        \hline
        TopicCoRank$_\textnormal{\textit{extr}}$ & 14.6 & 16.8 & 15.4$^{\dagger~~}$ & 36.4 & 24.6 & 28.7$^{~~~~}$ & 25.5 & 32.4 & 28.1$^{\dagger~~}$ & 15.2 & 10.6 & 12.4$^{\ddagger}$\\
        TopicCoRank$_\textnormal{\textit{assign}}$ & \textbf{24.9} & \textbf{28.9} & \textbf{26.4$^{\dagger\ddagger}$} & \textbf{49.1} & \textbf{33.3} & \textbf{38.8}$^{~~~~}$ & 25.9 & 33.3 & 28.8$^{\dagger~~}$ & 11.6 & ~~8.3 & ~~9.5$^{~~}$\\
        \hline
        TopicCoRank & 19.0 & 22.0 & 20.1$^{\dagger~~}$ & 39.5 & 26.6 & 31.1$^{~~~~}$ & \textbf{28.4} & \textbf{36.6} & \textbf{31.5$^{\dagger\ddagger}$} & \textbf{16.4} & \textbf{11.6} & \textbf{13.4$^{\ddagger}$}\\
        \bottomrule
      \end{tabular}
    }
    \caption{Comparison of TopicCoRank with the baselines. Precision (P), Recall
             (R) and F-score (F) are reported in percentages. $\dagger$ and $\ddagger$
             indicate a significant F-score improvement over, respectively, TopicRank and
             KEA++. \TODO{T-Test with KEA++}
             \label{tab:comparison_results}}
  \end{table*}
  Table~\ref{tab:comparison_results} summarizes the performance for three datasets of TopicCoRank,  TopicRank, and \textit{Assignment}, the keyphrase assignment baseline.
  The results show that \textit{Assignment} performs better than TopicRank on Inist and DUC datasets, to the contrary of
  SemEval. 
  %Results show the necessity, in some cases, to perform keyphrase assignment over keyphrase extraction.
  Keyphrase assignment seems to be more appropriate than keyphrase extraction for Inist and DUC text collections.
  %Based on observations from table~\ref{tab:corpus_statistics},  heterogeneously annotated are more difficult to treat by keyphrase assignment methods.
  Keyphrase extraction has to be preferred to keyphrase assignment for datasets such as SemEval that was heterogeneously annotated. 
  The main result is that TopicCoRank outperforms both TopicRank and \textit{Assignment} on all
  datasets. 
  
  Table~\ref{tab:comparison_results} shows the performance of two variants of TopicCoRank: TopicCoRank$_\textnormal{\textit{extr}}$ performs only  extraction
  and  TopicCoRank$_\textnormal{\textit{assign}}$ only assignment.
  The results of TopicCoRank$_\textnormal{\textit{extr}}$ and 
  TopicCoRank$_\textnormal{\textit{assign}}$ confirm that keyphrase assignment is more appropriate for 
  Inist and DUC, whereas keyphrase extraction is for SemEval.
  TopicCoRank outperforms TopicCoRank$_\textnormal{\textit{extr}}$ for all datasets.
  TopicCoRank outperforms TopicCoRank$_\textnormal{\textit{assign}}$ on DUC and SemEval, but not on Inist.
  
  %Inist contains so much missing keyphrases that domain keyphrases must be prioritized over document topics. 
  The Inist keyphrases are mainly missing keyphrases, i.e., domain keyphrases that do not occur in the bibliographic records. 
  For such dataset, domain keyphrases need to be prioritized over document topics. This could be done by giving more weight to the outer recommendation during the graph-based co-ranking.
  
  TopicCoRank and TopicCoRank$_\textnormal{\textit{extr}}$ outperform TopicCoRank$_\textnormal{\textit{assign}}$ for DUC and SemEval.
  The graph co-ranking algorithm successfully leverages document topics and
  controlled keyphrases to output both new concepts and appropriate controlled keyphrases.
  The new concepts that are identified could be used further to update domain-specific terminology.

  \ANNOTATE{Table~\ref{tab:assignment_ratio} shows the percentage of assigned keyphrases by TopicCoRank
  for each dataset. The statistics show that the co-ranking actually works and outputs both
  domain keyphrases and keyphrases from the document independently.}{Strengthen}
  \begin{table}[!h]
    \centering
    \begin{tabular}{l|c}
        \toprule
        & Assignment ratio\\
        \hline
        Linguistics & 38.7\%\\
        Archaeology & 32.2\%\\
        DUC & 58.6\%\\
        SemEval & 40.0\%\\
        \bottomrule
    \end{tabular}
    \caption{Percentage of assignment performed by TopicCoRank for 10 keyphrases
             \label{tab:assignment_ratio}}
  \end{table}
  
  To get a better understanding of the performance of each method, we plot
  precision-recall curves. Figure~\ref{fig:pr_curves1} shows the precision-recall curves
  of TopicRank, \textit{Assignment} and TopicCoRank for each dataset. 
  %Again, we can see that TopicCoRank outperforms the baselines. 
  TopicCoRank and TopicRank %have the same behavior. 
  behave similarly.  TopicCoRank is boosted by the keyphrase assignment. It achieves a better
  maximum precision and a better maximum recall.
  %boosted by keyphrase assignment. %Figure~\ref{fig:pr_curves2} shows the precision-recall
  %curves of TopicCoRank$_\textnormal{\textit{extr}}$,
  %TopicCoRank$_\textnormal{\textit{assign}}$ and TopicCoRank for each dataset. \TODO{\dots}
  \begin{figure*}
      \centering
      \subfigure[Linguistics]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0076038\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=40,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0076038\linewidth,
                       ytick={0, 10, 20, ..., 100},
                       ymin=0,
                       ymax=40,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/linguistique_topicrank.csv};
            \addplot [green, mark=-] file {input/data/linguistique_kea_pp.csv};
            \addplot [blue, mark=x] file {input/data/linguistique_topiccorank.csv};
            \addplot [dotted, domain=20:40] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:40] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:40] {(10 * x) / ((2 * x) - 10)};
            \legend{TopicRank, KEA++, TopicCoRank};
          \end{axis}
          \node at (4.9,3.1) [anchor=east] {\footnotesize{F=0.30}};
          \node at (4.9,1.8) [anchor=east] {\footnotesize{F=0.20}};
          \node at (4.9,0.9) [anchor=east] {\footnotesize{F=0.10}};
        \end{tikzpicture}
      }
      \subfigure[Archaeology]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0050692\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=60,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0050692\linewidth,
                       ytick={0, 15, 30, ..., 100},
                       ymin=0,
                       ymax=60,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/archeologie_topicrank.csv};
            \addplot [green, mark=-] file {input/data/archeologie_kea_pp.csv};
            \addplot [blue, mark=x] file {input/data/archeologie_topiccorank.csv};
            \addplot [dotted, domain=30:60] {(40 * x) / ((2 * x) - 40)};
            \addplot [dotted, domain=20:60] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:60] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:60] {(10 * x) / ((2 * x) - 10)};
            \legend{TopicRank, KEA++, TopicCoRank};
          \end{axis}
          \node at (4.9,2.65) [anchor=east] {\footnotesize{F=0.40}};
          \node at (4.9,1.85) [anchor=east] {\footnotesize{F=0.30}};
          \node at (4.9,1.15) [anchor=east] {\footnotesize{F=0.20}};
          \node at (4.9,0.65) [anchor=east] {\footnotesize{F=0.10}};
        \end{tikzpicture}
      }
      \subfigure[DUC]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0050692\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=60,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0050692\linewidth,
                       ytick={0, 15, 30, ..., 100},
                       ymin=0,
                       ymax=60,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/duc_topicrank.csv};
            \addplot [blue, mark=x] file {input/data/duc_topiccorank.csv};
            \addplot [dotted, domain=30:60] {(40 * x) / ((2 * x) - 40)};
            \addplot [dotted, domain=20:60] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:60] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:60] {(10 * x) / ((2 * x) - 10)};
            \legend{TopicRank, TopicCoRank};
          \end{axis}
          \node at (4.9,2.65) [anchor=east] {\footnotesize{F=0.40}};
          \node at (4.9,1.85) [anchor=east] {\footnotesize{F=0.30}};
          \node at (4.9,1.15) [anchor=east] {\footnotesize{F=0.20}};
          \node at (4.9,0.65) [anchor=east] {\footnotesize{F=0.10}};
        \end{tikzpicture}
      }
      \subfigure[SemEval]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0076038\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=40,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0076038\linewidth,
                       ytick={0, 10, 20, ..., 100},
                       ymin=0,
                       ymax=40,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/semeval_topicrank.csv};
            \addplot [blue, mark=x] file {input/data/semeval_topiccorank.csv};
            \addplot [dotted, domain=20:40] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:40] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:40] {(10 * x) / ((2 * x) - 10)};
            \legend{TopicRank, TopicCoRank};
          \end{axis}
          \node at (4.9,3.1) [anchor=east] {\footnotesize{F=0.30}};
          \node at (4.9,1.8) [anchor=east] {\footnotesize{F=0.20}};
          \node at (4.9,0.9) [anchor=east] {\footnotesize{F=0.10}};
        \end{tikzpicture}
      }
      \caption{Precision-recall curves of TopicRank, KEA++ and TopicCoRank
               for dataset
               \label{fig:pr_curves1}}
  \end{figure*}

  The influence of inner and outer recommendations with respect to the ranking is shown in  Figure~\ref{fig:lambda_variations}.
  The curves display the performance of TopicCoRank over the f-score with $\lambda$ ranging from $0.1$ to
  $0.9$.   We first observe that whatever is the value
  of $\lambda$, the worst performance of TopicCoRank is in the range of TopicRank
  performance. The keyphrase extraction is always improved by co-ranking. Secondly, a
  balanced influence nearly always induces the  best performances whatever is the dataset. TopicCoRank leverages
  both inner and outer recommendations. This means that controlled keyphrases and document topics
  can benefit from each other. We demonstrated the helpfulness of a co-ranking strategy for the automatic keyphrase
  annotation task.
  \begin{figure*}
      \centering
      \subfigure[Inist]{
        \begin{tikzpicture}[every axis/.append style={font=\tiny}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em, font=\small},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=14,
                       ymax=25,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em, font=\small}]
            \addplot[blue, mark=x] coordinates{
              (0.1, 20.04)
              (0.2, 20.22)
              (0.3, 20.37)
              (0.4, 20.14)
              (0.5, 20.09)
              (0.6, 18.46)
              (0.7, 16.69)
              (0.8, 15.98)
              (0.9, 16.43)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[DUC]{
        \begin{tikzpicture}[every axis/.append style={font=\tiny}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em, font=\small},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=24,
                       ymax=35,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em, font=\small}]
            \addplot[blue, mark=x] coordinates{
              (0.10, 31.96)
              (0.20, 32.24)
              (0.30, 32.40)
              (0.40, 31.92)
              (0.50, 31.53)
              (0.60, 30.50)
              (0.70, 28.23)
              (0.80, 26.61)
              (0.90, 24.63)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[SemEval]{
        \begin{tikzpicture}[every axis/.append style={font=\tiny}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em, font=\small},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=8,
                       ymax=19,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em, font=\small}]
            \addplot[blue, mark=x] coordinates{
              (0.10, 11.24)
              (0.20, 11.33)
              (0.30, 11.39)
              (0.40, 12.07)
              (0.50, 13.43)
              (0.60, 14.49)
              (0.70, 14.09)
              (0.80, 13.96)
              (0.90, 13.28)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \caption{Evolution of TopicCoRank's f-score (F) regarding the value of $\lambda$
               for each dataset
               \label{fig:lambda_variations}}
    \end{figure*}
    
    As already observed with results shown in table~\ref{tab:comparison_results}, the
    behavior of TopicCoRank differs between SemEval and the two other datasets. Values
    of $\lambda$ below $0.5$ induce better performances than those above $0.5$ on Inist and
    DUC, whereas the opposite observation raises from SemEval results. With a higher
    $\lambda$, the controlled graph highly influences the document topics and these topics obtain
    higher importance scores because the relations between topics are richer than
    between controlled keyphrases (more relations and higher weights). On Inist and DUC,
    artificially prioritizing keyphrase extraction with a higher $\lambda$ decreases
    the performance, whereas it increases the performance on SemEval.
    
    
  \begin{figure*}
      \centering
      \subfigure[Linguistic]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.349508\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.0,
                       xmax=1.0,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=14,
                       ymax=27,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.0, 15.42)
              (0.1, 16.56)
              (0.2, 17.23)
              (0.3, 17.73)
              (0.4, 18.54)
              (0.5, 19.56)
              (0.6, 20.78)
              (0.7, 22.31)
              (0.8, 23.85)
              (0.9, 25.29)
              (1.0, 26.18)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[Archaeology]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.349508\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.0,
                       xmax=1.0,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 40},
                       ymin=28,
                       ymax=41,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.0, 28.69)
              (0.1, 28.77)
              (0.2, 29.09)
              (0.3, 29.29)
              (0.4, 29.65)
              (0.5, 30.43)
              (0.6, 31.46)
              (0.7, 33.31)
              (0.8, 34.83)
              (0.9, 36.40)
              (1.0, 38.50)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[DUC]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.349508\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.0,
                       xmax=1.0,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 36},
                       ymin=24,
                       ymax=37,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.00, 28.15)
              (0.10, 29.97)
              (0.20, 30.95)
              (0.30, 32.15)
              (0.40, 33.00)
              (0.50, 32.86)
              (0.60, 32.34)
              (0.70, 31.59)
              (0.80, 30.99)
              (0.90, 30.29)
              (1.00, 29.44)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[SemEval]{
        \begin{tikzpicture}[every axis/.append style={font=\footnotesize}]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.349508\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.0,
                       xmax=1.0,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=8,
                       ymax=21,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.00, 12.36)
              (0.10, 13.04)
              (0.20, 0.0)
              (0.30, 13.56)
              (0.40, 0.0)
              (0.50, 12.79)
              (0.60, 12.68)
              (0.70, 11.50)
              (0.80, 11.06)
              (0.90, 10.78)
              (1.00, 9.69)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \caption{Evolution of TopicCoRank's f-score (F) regarding the assignment ratio
               for each dataset
               \label{fig:assignment_ratio_variations}}
    \end{figure*}

    \ANNOTATE{Finally, we provide insight into the improvement of TopicCoRank with an example of
    keyphrase annotation for the document \texttt{AP890708-0135} in DUC\footnote{A
    complete version of the document is available on the online AP news archive:
    \scriptsize\url{http://www.apnewsarchive.com/1989/Forests-Brush-Grass-Burn-In-The-Hot-Dry~-West/id-abcc43e9a37a9e5e1bf5ddfb4a3f0a17}.},
    namely \textit{Forests, Brush, Grass Burn In The Hot, Dry West}:
    \begin{center}
        \begin{varwidth}{.9\linewidth}
            \textbf{Reference}:
            \begin{enumerate*}
                \item{forest fire;}
                \item{firefighters;}
                \item{fire crews;}
                \item{fire lines;}
                \item{fire season;}
                \item{federal firefighting effort.}
            \end{enumerate*}
            \noindent\rule[0.5ex]{\linewidth}{.5pt}
            \textbf{TopicRank}:
            \begin{enumerate*}
                \item{fire;}
                \item{acres;}
                \item{miles;}
                \item{forest;}
                \item{wind;}
                \item{utah.}
            \end{enumerate*}\\
            \textbf{\textit{Assignment}}:
            \begin{enumerate*}
                \item{fire;}
                \item{forest;}
                \item{\underline{firefighters};}
                \item{utah;}
                \item{national forest;}
                \item{wyoming.}
            \end{enumerate*}\\
            \textbf{TopicCoRank}:
            \begin{enumerate*}
                \item{fire;}
                \item{\underline{firefighters};}
                \item{\underline{forest fire};}
                \item{\underline{fire lines};}
                \item{\underline{fire season};}
                \item{utah}.
            \end{enumerate*}
        \end{varwidth}
    \end{center}
    Underlined keyphrases correspond to correctly extracted and assigned keyphrases.}{Bad example}


==> attic/input/results2.tex <==
\section{Results}
\label{sec:results}
    \begin{figure*}
      \centering
      \subfigure[Linguistics]{
        \begin{tikzpicture}[scale=.5925]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0076038\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=40,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0076038\linewidth,
                       ytick={0, 10, 20, ..., 100},
                       ymin=0,
                       ymax=40,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/linguistique_topicrank.csv};
            \addplot [green, mark=o] file {input/data/linguistique_kea_pp.csv};
            \addplot [blue, mark=x] file {input/data/linguistique_topiccorank.csv};
            \addplot [dotted, domain=20:40] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:40] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:40] {(10 * x) / ((2 * x) - 10)};
            %\legend{TopicRank, KEA++, TopicCoRank};
          \end{axis}
          \node at (4.9,3.1) [anchor=east] {\scriptsize{F=30.0}};
          \node at (4.9,1.8) [anchor=east] {\scriptsize{F=20.0}};
          \node at (4.9,0.9) [anchor=east] {\scriptsize{F=10.0}};
        \end{tikzpicture}
      }
      \subfigure[Archaeology]{
        \begin{tikzpicture}[scale=.5925]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0050692\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=60,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0050692\linewidth,
                       ytick={0, 15, 30, ..., 100},
                       ymin=0,
                       ymax=60,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/archeologie_topicrank.csv};
            \addplot [green, mark=o] file {input/data/archeologie_kea_pp.csv};
            \addplot [blue, mark=x] file {input/data/archeologie_topiccorank.csv};
            \addplot [dotted, domain=30:60] {(40 * x) / ((2 * x) - 40)};
            \addplot [dotted, domain=20:60] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:60] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:60] {(10 * x) / ((2 * x) - 10)};
            %\legend{TopicRank, KEA++, TopicCoRank};
          \end{axis}
          \node at (4.9,2.65) [anchor=east] {\scriptsize{F=40.0}};
          \node at (4.9,1.85) [anchor=east] {\scriptsize{F=30.0}};
          \node at (4.9,1.15) [anchor=east] {\scriptsize{F=20.0}};
          \node at (4.9,0.65) [anchor=east] {\scriptsize{F=10.0}};
        \end{tikzpicture}
      }
      \subfigure[DUC]{
        \begin{tikzpicture}[scale=.5925]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0050692\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=60,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0050692\linewidth,
                       ytick={0, 15, 30, ..., 100},
                       ymin=0,
                       ymax=60,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\footnotesize}]
            \addplot [red, mark=+] file {input/data/duc_topicrank.csv};
            \addplot [blue, mark=x] file {input/data/duc_topiccorank.csv};
            \addplot [dotted, domain=30:60] {(40 * x) / ((2 * x) - 40)};
            \addplot [dotted, domain=20:60] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:60] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:60] {(10 * x) / ((2 * x) - 10)};
            %\legend{TopicRank, TopicCoRank};
          \end{axis}
          \node at (4.9,2.65) [anchor=east] {\scriptsize{F=40.0}};
          \node at (4.9,1.85) [anchor=east] {\scriptsize{F=30.0}};
          \node at (4.9,1.15) [anchor=east] {\scriptsize{F=20.0}};
          \node at (4.9,0.65) [anchor=east] {\scriptsize{F=10.0}};
        \end{tikzpicture}
      }
      \subfigure[SemEval]{
        \begin{tikzpicture}[scale=.5925]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.0076038\linewidth,
                       xtick={0, 20, 40, ..., 100},
                       xmin=0,
                       xmax=40,
                       xlabel=recall (\%),
                       x label style={yshift=.34em},
                       y=0.0076038\linewidth,
                       ytick={0, 10, 20, ..., 100},
                       ymin=0,
                       ymax=40,
                       ylabel=precision (\%),
                       y label style={yshift=-1.1em},
                       legend style={font=\Large}]
            \addplot [red, mark=+] file {input/data/semeval_topicrank.csv};
            \addplot [green, mark=o] coordinates {
                (-1.0, -1.0)
            };
            \addplot [blue, mark=x] file {input/data/semeval_topiccorank.csv};
            \addplot [dotted, domain=20:40] {(30 * x) / ((2 * x) - 30)};
            \addplot [dotted, domain=10:40] {(20 * x) / ((2 * x) - 20)};
            \addplot [dotted, domain=5:40] {(10 * x) / ((2 * x) - 10)};
            \legend{TopicRank, KEA++, TopicCoRank};
          \end{axis}
          %\node at (4.9,3.1) [anchor=east] {\scriptsize{F=30.0}};
          \node at (4.9,1.8) [anchor=east] {\scriptsize{F=20.0}};
          \node at (4.9,0.9) [anchor=east] {\scriptsize{F=10.0}};
        \end{tikzpicture}
      }
      \caption{Precision-recall curves of TopicRank, KEA++ and TopicCoRank
               for each dataset
               \label{fig:pr_curves1}}
    \end{figure*}
    
    \begin{figure*}
      \centering
      \subfigure[Linguistics]{
        \begin{tikzpicture}[scale=.525]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.00349508\linewidth,
                       xtick={0, 20, ..., 100},
                       xmin=0.0,
                       xmax=100.0,
                       xlabel=Assignment ratio (\%),
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=14,
                       ymax=28,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0, 15.42)
              (10, 16.56)
              (20, 17.23)
              (30, 17.73)
              (40, 18.54)
              (50, 19.56)
              (60, 20.78)
              (70, 22.31)
              (80, 23.85)
              (90, 25.29)
              (100, 26.18)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[Archaeology]{
        \begin{tikzpicture}[scale=.525]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.00349508\linewidth,
                       xtick={0, 20, ..., 100},
                       xmin=0.0,
                       xmax=100.0,
                       xlabel=Assignment ratio (\%),
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 42},
                       ymin=28,
                       ymax=42,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0, 28.69)
              (10, 28.77)
              (20, 29.09)
              (30, 29.29)
              (40, 29.65)
              (50, 30.43)
              (60, 31.46)
              (70, 33.31)
              (80, 34.83)
              (90, 36.40)
              (100, 38.50)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[DUC]{
        \begin{tikzpicture}[scale=.525]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.00349508\linewidth,
                       xtick={0, 20, ..., 100},
                       xmin=0.0,
                       xmax=100.0,
                       xlabel=Assignment ratio (\%),
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 38},
                       ymin=24,
                       ymax=38,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0, 28.15)
              (10, 29.97)
              (20, 30.95)
              (30, 32.15)
              (40, 33.00)
              (50, 32.86)
              (60, 32.34)
              (70, 31.59)
              (80, 30.99)
              (90, 30.29)
              (100, 29.44)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[SemEval]{
        \begin{tikzpicture}[scale=.525]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.00349508\linewidth,
                       xtick={0, 20, ..., 100},
                       xmin=0.0,
                       xmax=100.0,
                       xlabel=Assignment ratio (\%,
                       x label style={yshift=.34em},
                       y=0.016675\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=8,
                       ymax=22,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0, 12.36)
              (10, 13.04)
              (20, 13.72)
              (30, 13.56)
              (40, 13.43)
              (50, 12.79)
              (60, 12.68)
              (70, 11.50)
              (80, 11.06)
              (90, 10.78)
              (100, 9.69)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \caption{Behavior of TopicCoRank's f-score (F) regarding the assignment ratio
               for each dataset
               \label{fig:assignment_ratio_variations}}
    \end{figure*}
    
    Table~\ref{tab:comparison_results} shows the results obtained with
    TopicCoRank and the baselines for each of the datasets. Overall, we observe that TopicCoRank significantly outperforms TopicRank and KEA++. Surprisingly, KEA++  achieves low performance. The main reason is that a large proportion of the controlled keyphrases do not occur within the documents ($\simeq$50\%). We also observed that the thesauri we use, which are real case scenario thesauri, contain less semantic relations than the one applied by \newcite{medelyan2006kea++} on random documents from the UN Food and Agriculture Organization (FAO). Concerning TopicCoRank and its variants, TopicCoRank performs better on DUC and SemEval, while its assignment variant, TopicCoRank$_\textnormal{\textit{assign}}$, performs better on Linguistics and Archaeology. The annotation strategy of the professional indexers is centered on controlled vocabularies, which explains why the assignment should be prioritized on the case of Linguistics and Archaeology. However, by better performing, TopicCoRank$_\textnormal{\textit{assign}}$ shows that the ranking of the controlled keyphrases efficiently gives importance to the controlled keyphrases in the context of the document. Therefore, connecting document topics to controlled keyphrases is useful for the ranking.

    Moreover, the results we observe on DUC are highly competitive with the best reported
    results on DUC (31.7\% of f-score)~\cite{wan2008expandrank} and higher than the best
    reproduced results (26.4\% of f-score)~\cite{hassan2010conundrums}.
  
    Precision-recall curves displayed in figure~\ref{fig:pr_curves1}, confirms the
    previous observations. In term of optimizing precision and recall, TopicCoRank
    dominates both TopicRank and KEA++, which means that TopicCoRank achieves the
    best performance for any precision and recall values.
  
    Table~\ref{tab:assignment_ratio} shows the percentage of keyphrases assigned by
    TopicCoRank at 10 keyphrases for each dataset. As we claimed, the percentage of assigned keyphrases per document shows that TopicCoRank independently assigns and extracts keyphrases. 
    \begin{table}[!h]
        \centering
        \begin{tabular}{l|c}
            \toprule
            & Assignment ratio\\
            \hline
            Linguistics & 38.7\%\\
            Archaeology & 32.2\%\\
            DUC & 58.6\%\\
            SemEval & 40.0\%\\
            \bottomrule
        \end{tabular}
        \caption{Average ratio of assignment performed by TopicCoRank at 10 keyphrases
                 \label{tab:assignment_ratio}}
    \end{table}
    
    \begin{figure*}
      \centering
      \subfigure[Linguistics]{
        \begin{tikzpicture}[scale=.7425]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=14,
                       ymax=26,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.1, 20.04)
              (0.2, 20.22)
              (0.3, 20.37)
              (0.4, 20.14)
              (0.5, 20.09)
              (0.6, 18.46)
              (0.7, 16.69)
              (0.8, 15.98)
              (0.9, 16.43)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[Archaeology]{
        \begin{tikzpicture}[scale=.7425]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 36},
                       ymin=24,
                       ymax=36,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.1, 32.20)
              (0.2, 31.74)
              (0.3, 31.58)
              (0.4, 31.33)
              (0.5, 31.09)
              (0.6, 30.64)
              (0.7, 28.96)
              (0.8, 26.52)
              (0.9, 24.61)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[DUC]{
        \begin{tikzpicture}[scale=.7425]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 36},
                       ymin=24,
                       ymax=36,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.10, 31.96)
              (0.20, 32.24)
              (0.30, 32.40)
              (0.40, 31.92)
              (0.50, 31.53)
              (0.60, 30.50)
              (0.70, 28.23)
              (0.80, 26.61)
              (0.90, 24.63)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \subfigure[SemEval]{
        \begin{tikzpicture}[scale=.7425]
          \pgfkeys{/pgf/number format/.cd, fixed}
          \begin{axis}[x=0.262\linewidth,
                       xtick={0.1, 0.3, ..., 0.9},
                       xmin=0.05,
                       xmax=0.95,
                       xlabel=$\lambda$,
                       x label style={yshift=.34em},
                       y=0.0125\textheight,
                       ytick={0, 2, 4, ..., 34},
                       ymin=8,
                       ymax=20,
                       ylabel=f-score (\%),
                       y label style={yshift=-1.1em}]
            \addplot[blue, mark=x] coordinates{
              (0.10, 11.24)
              (0.20, 11.33)
              (0.30, 11.39)
              (0.40, 12.07)
              (0.50, 13.43)
              (0.60, 14.49)
              (0.70, 14.09)
              (0.80, 13.96)
              (0.90, 13.28)
            };
          \end{axis}
        \end{tikzpicture}
      }
      \caption{Behavior of TopicCoRank's f-score (F) regarding the value of $\lambda$
               for each dataset
               \label{fig:lambda_variations}}
    \end{figure*}

    Furthermore, we artificially vary the assignment ratio and show the resulting performances of TopicCoRank in figure~\ref{fig:assignment_ratio_variations}. Results also show the difference between the two Linguistics and Archaeology datasets and the two DUC and SemEval datasets. On Linguistics and Archaeology, the performance of TopicCoRank is in the form of a pseudo-cumulative curve: the more TopicCoRank assigns, the better it performs. On DUC and SemEval, the performance of TopicCoRank is in the form of a pseudo-normal curve: extraction and assignment must be balanced to achieve better results.
    Linguistics and Archaeology have been annotated with a strong focus on controlled vocabulary, which explains why assignment should be prioritized. DUC and SemEval have been freely annotated. In that case, the default TopicCoRank, which tends to balance assignment and extraction, achieves a near optimal performance.
    
    Additionally, figure~\ref{fig:lambda_variations} shows the behavior of TopicCoRank
    regarding the value of $\lambda$, which configures the importance of the inner
    recommendation over the outer recommendation. Globally, we can see that balancing
    the recommendation between the inner and the outer recommendation induces
    near-optimal performances. This observation indicates that the specific domain of a
    document is as important as the content of the document.
    
    Finally, we provide insights of the improvement of TopicCoRank over TopicRank with
    an example of keyphrase annotation for the document \texttt{FT941-1547} of DUC, namely
    \textit{Commodities and Agriculture: Germany sets scientist to work}, which talks about
    a German research project to examine whether the cattle disease bovine spongiform
    encephalopathy (BSE) can be transmitted to human beings:
    \begin{center}
        \begin{varwidth}{.9\linewidth}
            \textbf{Reference}:
            \begin{enumerate*}
                \item{cattle disease;}
                \item{bovine spongiform encephalopathy;}
                \item{BSE;}
                \item{mad cow disease;}
                \item{British beef imports;}
                \item{possible connections.}
            \end{enumerate*}
            \noindent\rule[0.5ex]{\linewidth}{.5pt}
            \textbf{TopicRank}:
            \begin{enumerate*}
                \item{\underline{British beef imports};}
                \item{human beings;}
                \item{new research project;}
                \item{disease;}
                \item{non-existent;}
                \item{German universities.}
            \end{enumerate*}\\
            \textbf{TopicCoRank}:
            \begin{enumerate*}
                \item{\underline{British beef imports};}
                \item{\underline{BSE};}
                \item{\underline{mad cow disease};}
                \item{ban;}
                \item{\underline{bovine spongiform encephalopathy};}
                \item{Germany.}
            \end{enumerate*}
        \end{varwidth}
    \end{center}
    Underlined keyphrases correspond to correctly extracted and assigned keyphrases.


==> attic/input/topicrankpp.tex <==
\section{Co-ranking for Keyphrase Annotation}
\label{sec:topicrankpp}

  This section presents TopicCoRank\footnote{TopicCoRank will soon be publicly available on GitHub.}, our keyphrase annotation method.
  We first describe TopicRank~\cite{bougouin2013topicrank}, the 
  graph-based ranking approach to keyphrase extraction on which we build.
  We then present our unified graph model, and the co-ranking
  strategy we propose for performing both keyphrase extraction and assignment.
  
  \subsection{TopicRank}
  \label{subsec:topicrank}
    TopicRank is an unsupervised graph-based method that topically clusters the
    keyphrase candidates of a document, ranks the topics (topical clusters) and extracts the
    most representative keyphrase for each of the $N$ most important topics. It
    relies on four main steps: topical clustering, graph construction,
    graph-based topic ranking and extraction of the most representative keyphrase
    per topic.
    
    Sequences of adjacent words restricted to nouns and adjectives (\texttt{/(N|A)+/}) are 
    considered as keyphrase candidates.
    In TopicRank, similar keyphrase candidates are clustered into topics based
    on the words they share.
    \newcite{bougouin2013topicrank} use a Hierarchical
    Agglomerative Clustering (HAC) with a stem overlap similarity (see equation~\ref{math:jaccard}) and an average linkage: at
    the beginning, each keyphrase candidate is a single cluster, then candidates
    sharing an average of $\unitfrac{1}{4}$ stemmed words with the candidates of
    another cluster are iteratively added to the latter.
    \begin{align}
      \text{sim}(v_i, v_j) &= \frac{|\text{stems}(v_i) \cap \text{stems}(v_j)|}{|\text{stems}(v_i) \cup \text{stems}(v_j)|} \label{math:jaccard}
    \end{align}
    
    A complete graph is built, in which nodes are topics and edges are weighted according to the strength of the semantic
    relation between the connected topics. The closer two topics occur in the
    document, the stronger is their semantic relation.
    
    The importance ranking of the topics is performed with TextRank, modified to exploit edge
    weights $w$~\cite{wan2008expandrank} (see equation~\ref{math:singlerank}).
    \begin{align}
      S(v_i) = (1 - \lambda) + \lambda \sum_{v_j \in E(v_i)}{\frac{w_{ij}S(v_j)}{\mathlarger\sum_{v_k \in E(v_j)}{w_{jk}}}}\label{math:singlerank}
    \end{align}
      
    The keyphrase extraction is performed on the $N$  most important topics. To
    avoid topic redundancy, only one
    keyphrase per topic is extracted.
    Following previous observations~\cite{witten1999kea},
    the first occurring keyphrase candidate is chosen.

  \subsection{Graph construction for co-ranking}
  \label{subsec:graph_construction}
    TopicCoRank operates over a unified graph that connects two graphs
    representing the controlled keyphrases, the document topics and
    the relations between them. Controlled keyphrases are keyphrases
    that were manually assigned to training documents. We consider the 
    controlled keyphrases
    to be our controlled vocabulary for the keyphrase assignment.
    As controlled keyphrases are presumably non-redundant, we do not 
    group them by topics as we do for keyphrase candidates.
    
    Let
    $G = (V, E=E_{\textnormal{\textit{in}}} \cup E_{\textnormal{\textit{out}}})$
    denote the unified graph. Controlled keyphrases and topics are vertices $V$
    connected to their fellows by edges $E_\textnormal{\textit{in}}$ and
    connected to the other vertices by edges $E_\textnormal{\textit{out}}$ (see
    Figure~\ref{fig:topicrankpp_graph})\footnote{$E_\textnormal{\textit{in}} \subset V \times V$, $E_\textnormal{\textit{out}} \subset V \times V$, and $E_\textnormal{\textit{in}} \cup E_\textnormal{\textit{out}} = \emptyset$.}.
    
    \begin{figure*}
      \newcommand{\xslant}{0.25}
      \newcommand{\yslant}{0}

      \centering
      \begin{tikzpicture}[transform shape, scale=.667]
        % frame
        \node [draw,
               rectangle,
               minimum width=.9\linewidth,
               minimum height=7em,
               xslant=\xslant,
               yslant=\yslant] (domain_graph) {};
        \node [above=of domain_graph,
               xshift=.45\linewidth,
               yshift=7em,
               anchor=south east] (domain_graph_label) {controlled keyphrases};

        \node [draw,
               circle,
               above=of domain_graph,
               xshift=.3\linewidth,
               yshift=4em] (domain_node1) {$v_1$};
        \node [draw,
               circle,
               above=of domain_graph,
               xshift=-.3\linewidth,
               yshift=4em] (domain_node2) {$v_2$};
        \node [draw,
               circle,
               above=of domain_graph,
               yshift=4em] (domain_node3) {$v_3$};
        \node [draw,
               circle,
               above=of domain_graph,
               xshift=.15\linewidth,
               yshift=.75em] (domain_node4) {$v_4$};
        \node [draw,
               circle,
               above=of domain_graph,
               xshift=-.15\linewidth,
               yshift=.75em] (domain_node5) {$v_5$};

        \draw (domain_node1) -- (domain_node3);
        \draw (domain_node2) -- (domain_node3);
        \draw (domain_node2) -- (domain_node4);
        \draw (domain_node4) -- (domain_node5);
        \draw (domain_node4) -- (domain_node3);

        % document
        \node [draw,
               rectangle,
               minimum width=.9\linewidth,
               minimum height=7em,
               xslant=\xslant,
               yslant=\yslant,
               above=of domain_graph,
               xshift=-2em] (document_graph) {};
        \node [below=of document_graph,
               xshift=-.45\linewidth,
               yshift=-7em,
               anchor=north west] (document_graph_label) {document topics};

        \node [draw,
               circle,
               below=of document_graph,
               xshift=.3\linewidth,
               yshift=-4em] (document_node1) {$v_6$};
        \node [draw,
               circle,
               below=of document_graph,
               xshift=-.3\linewidth,
               yshift=-4em] (document_node2) {$v_7$};
        \node [draw,
               circle,
               below=of document_graph,
               yshift=-4em] (document_node3) {$v_8$};
        \node [draw,
               circle,
               below=of document_graph,
               xshift=.15\linewidth,
               yshift=-.75em] (document_node4) {$v_9$};

        \draw (document_node2) -- (document_node3);
        \draw (document_node3) -- (document_node1);
        \draw (document_node1) -- (document_node4);
        \draw (document_node3) -- (document_node4);

        % extra link
        \draw [dashed] (document_node2) -- (domain_node2);
        \draw [dashed] (document_node3) -- (domain_node3);
        \draw [dashed] (document_node4) -- (domain_node1);
        \draw [dashed] (document_node3) -- (domain_node4);

        % legend
        \node [right=of document_graph, xshift=2em, yshift=-8em] (legend_title) {\underline{Legend:}};
        \node [below=of legend_title, xshift=-1em, yshift=2em] (begin_inner) {};
        \node [right=of begin_inner] (end_inner) {: $E_\textnormal{\textit{in}}$};
        \node [below=of begin_inner, yshift=1.5em] (begin_outer) {};
        \node [right=of begin_outer] (end_outer) {: $E_\textnormal{\textit{out}}$};

        \draw (legend_title.north  -| end_outer.east) rectangle (end_outer.south -| legend_title.west);

        \draw (begin_inner) -- (end_inner);
        \draw [dashed] (begin_outer) -- (end_outer);
      \end{tikzpicture}
      \caption{Example of a unified graph constructed by TopicCoRank and its two
               kinds of edges
               \label{fig:topicrankpp_graph}}
    \end{figure*}

    To unify the two graphs, we consider the controlled keyphrases as a category map and connect the document to its potential categories. We create an edge
    $\langle{}v_i, v_j\rangle{} \in E_{\textnormal{\textit{out}}}$ to connect a controlled
    keyphrase $v_i$ and a topic $v_j$ if the controlled keyphrase is a
    member of the topic, i.e., a keyphrase candidate in the topic.
    To accept flexions, such as plural flexions, we perform the comparison with
    stems.
    We create an edge $\langle{}v_i, v_j\rangle{} \in E_\textnormal{\textit{in}}$ between two controlled
    keyphrases or two topics $v_i$ and $v_j$ when they co-occur, respectively, as keyphrases of
    a training document or within a sentence of the
    document. Each edge $\langle{}v_i, v_j\rangle{} \in E_{\textnormal{\textit{in}}}$ is weighted by
    the normalized number of co-occurrences $w_{ij}$ of the controlled
    keyphrases or the topics $v_i$ and $v_j$ within the keyphrase sets of each training document or the document, respectively. The weighting scheme of edges
    $E_\textnormal{\textit{in}}$ is equivalent for both controlled keyphrases and
    topics. This equivalence is essential to properly co-rank controlled keyphrases
    and topics and, therefore, ensure that not only controlled keyphrases occurring in the document can be assigned.

  \subsection{Graph-based co-ranking}
  \label{subsec:graph_based_co_ranking}
    TopicCoRank gives an importance score $S(v_i)$ to every vertex
    $v_i$ using graph co-ranking (see equation~\ref{math:topiccorank}).
    Graph co-ranking has been applied with success to many NLP tasks 
    such as text summarization~\cite{wan2011corankingsummarization}, 
    tweet recommendation~\cite{yan2012corankingtweetrecommendation} or 
    opinion mining~\cite{liu2014corankingopinionmining}.
    
    The
    graph co-ranking simulates the ``voting concept'' based on inner and outer
    recommendations. The inner recommendation $R_\textnormal{\textit{in}}$ of a
    node comes from nodes of the same graph (see equation~\ref{math:rin}):
    \begin{itemize}
      \item{a controlled keyphrase is important if it is strongly connected to other
            controlled keyphrases;}
      \item{a topic is important if it is strongly connected to other topics.}
    \end{itemize}
    The outer recommendation $R_\textnormal{\textit{out}}$ of a node comes from nodes
    of the other graph (see equation~\ref{math:rout}):
    \begin{itemize}
      \item{a controlled keyphrase is more important in the context of the document if it
            is connected to one of its important topics;}
      \item{a topic is more important if it is connected to important controlled keyphrases.}
    \end{itemize}
    \begin{align}
      S(v_i) &= (1 - \lambda)\ R_{out}(v_i) + \lambda\ R_{in}(v_i)\label{math:topiccorank}\\
      R_{in}(v_i) &= \sum_{v_j \in E_{\text{in}}(v_i)}{\frac{w_{ij} S(v_j)}{\mathlarger\sum_{v_k \in E_{\text{in}}(v_j)}{{w_{jk}}}}}\label{math:rin}\\
      R_{out}(v_i) &= \sum_{v_j \in E_{\text{out}}(v_i)}{\frac{S(v_j)}{|E_{\text{\textit{out}}}(v_j)|}}\label{math:rout}
    \end{align}
    $\lambda$ is a parameter that controls the influence of the inner recommendation
    over the outer recommendation ($0 \leq \lambda \leq 1$). A higher $\lambda$
    gives more influence to the inner recommendation and a lower $\lambda$ gives
    more influence to the outer recommendation. By default, we set $\lambda$ to $0.5$
    to give the same impact to both recommendations.

    \begin{table*}
      \centering
      %\resizebox{.8\linewidth}{!}{
          \begin{tabular}{l|cccc|cc}
            \toprule
            \multirow{2}{*}{\textbf{Corpus}} & \multicolumn{4}{c|}{\textbf{Documents}} & \multicolumn{2}{c}{\textbf{Keyphrases}}\\
            \cline{2-7}
            & Type & Language & Number & Tokens average & Average & Missing\\
            \hline
            Linguistics & & & & & &\\
            $\drsh$~train & Abstracts & French & 515 & $~~$161 & $~~$8.6 & 60.6\%\\
            $\drsh$~test & Abstracts & French & 200 & $~~$147 & $~~$8.9 & 62.8\% \\
            \hline
            Archaeology & & & & & &\\
            $\drsh$~train & Abstracts & French & 518 & $~~$221 & 16.9 & 37.0\%\\
            $\drsh$~test & Abstracts & French & 200 & $~~$214 & 15.6 & 37.4\%\\
            \hline
            DUC & News & English & 308 & $~~$901 & $~~$8.1 & $~~$3.5\%\\
            \hline
            SemEval & & & & & &\\
            $\drsh$~train & Papers & English & 144 & 5135 & 15.4 & 13.5\%\\
            $\drsh$~test & Papers & English & 100 & 5178 & 14.7 & 22.1\%\\
            \bottomrule
          \end{tabular}
      %}
      \caption{Dataset statistics. ``Missing'' represents the percentage of keyphrases
               that cannot be retrieved within the documents.
               \label{tab:corpus_statistics}}
    \end{table*}

  \subsection{Keyphrase annotation}
  \label{subsec:keyphrase_assignment_and_extraction}
    To both assign and extract keyphrases, we sort the controlled
    keyphrases and the topics based on their importance score $S$. The $N$-best ranking ones are
    considered as the keyphrases of the document regardless of their nature (topic keyphrase or controlled keyphrase).

    We assign controlled keyphrases over one condition. A controlled keyphrase can
    be assigned to a document if it is directly or transitively connected to a
    topic of the document. Indeed, if the ranking of a controlled keyphrase has not been
    affected by topics of the document nor controlled keyphrases connected to topics,
    its importance score is not related to the content of the document and we do not
    want to assign them.

    We extract keyphrases from the topics using the former TopicRank strategy.
    Only one keyphrase is extracted per topic: the
    candidate that occurs first within the document.


==> input/data/conclusion-v2.tex <==
\section{Conclusion}
\label{sec:conclusion}
     In this paper, we have proposed a co-ranking approach to performing keyphrase
  extraction and keyphrase assignment jointly. Our method,
  TopicCoRank, builds two graphs: one with the
  document topics and one with controlled keyphrases (training keyphrases). We
  design a strategy to unify the two graphs and rank by importance topics and
  controlled keyphrases using a co-ranking vote.
  We performed experiments on three French datasets of  humanities:  linguistics, information science and archaeology. Results showed that our approach benefits from both controlled
  keyphrases and document topics, improving both keyphrase extraction and keyphrase assignment
  baselines. TopicCoRank can be used to annotate keyphrases in scientific domains in a close way of profession l indexers do it.
    
    %
    Of course,   TopicCoRank still suffers from limitations that are shared by many keyphrase extraction and assignment methods.  Our keyphrase extraction method adopts a ``naive'' topical clustering that may be replaced by a more sophisticated one in order to build more reliable concept clusters gathering all keyphrase variants.  The keyphrase assignment method uses as training data the pre-assigned keywords of scientific documents belonging to the same domain. Other  unsupervised constructions of the domain graph (using Wikipedia data, bootstrapping techniques, etc.) could be explored as well as  more complex unification strategies in order to more accurately connect the document and the domain graph.



